Deep Structural Knowledge Exploitation and Synergy for Estimating Node Importance Value on Heterogeneous Information Networks

Node importance estimation problem has been studied conventionally with homogeneous network topology analysis. To deal with network heterogeneity, a few recent methods employ graph neural models to automatically learn diverse sources of information. However, the major concern revolves around that their full adaptive learning process may lead to insufficient information exploration, thereby formulating the problem as the isolated node value prediction with underperformance and less interpretability. In this work, we propose a novel learning framework: SKES. Different from previous automatic learning designs, SKES exploits heterogeneous structural knowledge to enrich the informativeness of node representations. Based on a sufficiently uninformative reference, SKES estimates the importance value for any input node, by quantifying its disparity against the reference. This establishes an interpretable node importance computation paradigm. Furthermore, SKES dives deep into the understanding that "nodes with similar characteristics are prone to have similar importance values" whilst guaranteeing that such informativeness disparity between any different nodes is orderly reflected by the embedding distance of their associated latent features. Extensive experiments on three widely-evaluated benchmarks demonstrate the performance superiority of SKES over several recent competing methods.

==> sections/tables/centrality.tex <==
\begin{table*}[t]
\fontsize{8}{9} \selectfont
\centering
\caption{Definitions of nine representative centrality measures.}
\vspace{-8pt}
\label{tab:centralityFormula}
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{ >{\raggedright\arraybackslash}p{0.35\linewidth}| >{\raggedright\arraybackslash}p{0.6\linewidth} }
\specialrule{.1em}{0em}{0em}
    {\bf Centrality measure}&
    {\bf Definition}\\
    \specialrule{.1em}{0em}{0em}
    
    Degree centrality \cite{nieminen1974centrality}&
    $c_{i}^{(1)} = \sum_{j=1}^N a_{ij} $, where $N$ is the number of nodes, and $\mathbf A$=$(a_{ij})$ is the adjacency matrix.\\
    \hline

    Eigenvector centrality \cite{bonacich2007some}
    &
    \tabincell{l}{
       $c_{i}^{(2)}=\lambda\sum_{j=1}^N a_{ij}x_{j}$, where $\lambda$ and $\mathbf x$ are the largest eigenvalue and corresponding\\eigenvector of $\mathbf A$, respectively, i.e., $\mathbf x=\lambda \mathbf A \mathbf x$. $x_j$ is the $j$-th element of $\mathbf x$.
    }\\
    \hline
    
    Harmonic centrality \cite{marchiori2000harmony}&
    $c_{i}^{(3)}=\sum_{j=1, j \neq i}^N 1/d(j,i)$, where $d(j,i)$ is the distance between nodes $j$ and $i$.\\
    \hline
    
    Closeness centrality \cite{sabidussi1966centrality}&
    $c_{i}^{(4)}=(N-1)/\sum_{j=1, j\neq i}^N d(j,i).$ %where $d(j,i)$ is the distance between nodes $j$ and $i$, and N is the number of nodes in graph.
    \\                       
    \hline
    
    Betweenness centrality \cite{bader2007approximating}
    &
    \tabincell{l}{
        $c_{i}^{(5)}=\sum_{s\neq i \neq t \in [1,N] } \sigma_{st}(i)/\sigma_{st}$, where $\sigma_{st}$ is total number of shortest paths from \\node $s$ to node $t$, and $\sigma_{st}(i)$ is the number of paths that pass through node $i$.
    }
    \\
    \hline
    
    Pagerank centrality \cite{page1999pagerank}&
    \makecell[l]{$c_{i}^{(6)}=\gamma \sum_{j=1}^N a_{ji}c_{j}^{(6)}/c_j^{(1)}+ (1-\gamma)/N$, where $\gamma$ is the damping factor. %\\ \cmtchn{alpha与后续变量冲突，更换一下，并指明这是一个常数} 
    }\\
    \hline
    
    Coreness centrality \cite{bae2014identifying}&
    $c_{i}^{(7)}=\sum_{j=1}^N a_{ij}ks(j)$, where $ks(j)$ is the $k$-shell index of its neighbor node $j$.\\
    \hline
    
    H-index centrality \cite{hirsch2005index}&
    One node's h-index is $h$, if it has $h$ neighbors, each of which has a degree of at least $h$. \\
    \hline
    
    G-index centrality \cite{egghe2006improvement}&
    It is the largest number of $g$ neighbors for which the average degree is at least $g^2$.\\
    \specialrule{.1em}{0em}{0em}
\end{tabular}
}
\end{table*}

==> sections/tables/hyperparameter.tex <==
\begin{table}[t]
\fontsize{8}{9} \selectfont
\centering
\caption{Hyperparameter settings for all datasets.}
\vspace{-8pt}
\label{tab:setting}
\setlength{\tabcolsep}{0.7mm}{
	\begin{tabular}{c|p{2cm}<{\centering} |p{2cm}<{\centering} |p{2cm}<{\centering} }
	\specialrule{.1em}{0em}{0em}
	Hyperparameter  & MUSIC10K  & TMDB5K  & DBLP                                                                                                                 \\ \specialrule{.1em}{0em}{0em}
	$M$       & 8  & 8 & 8   \\ \cline{1-4}
	$d$ 		& 256  & 256 & 256   \\ \cline{1-4}
	$R$			& 4  & 6 & 4   \\ \cline{1-4}
	$lr$		& 0.001	& 0.001	& 0.001 \\ \cline{1-4}
	$\mu$		&0.0001	&0.0001	&0.0001 \\ \specialrule{.1em}{0em}{0em}
	

	\end{tabular}
}
\end{table}
% consider to simply it!



==> sections/tables/metapaths.tex <==

\begin{table}[t]
\fontsize{8}{9} \selectfont
\centering
\setlength{\tabcolsep}{1.7mm}{
	\begin{tabular}{c|p{2.5cm}<{\centering}|p{3.5cm}<{\centering}}
	\specialrule{.1em}{0em}{0em}
	Dataset  & Node type  & Meta-paths                                                                                                                                                                                                                      \\ \specialrule{.1em}{0em}{0em}
	\multirow{4}{*}{MUSIC10K} & Song (S)  & SAS, SATAS, SRARS \\ \cline{2-3}
	                          & Arist (A) & ATA, ARA, ASA  \\ \cline{2-3}
	                          & Term (T)  & TAT, TASAT, TARAT \\ \cline{2-3}
	                          & Release(R)& RSR, RAR, RSASR  \\ \hline


	\multirow{7}{*}{TMDB5K}   & Movie (M)    & MDM, MCM, MPM \\ \cline{2-3}
	                          & Cast (C)     & CMC, CMDMC, CMPMC \\ \cline{2-3}
	                          & Director (D) & DMD, DMCMD, DMPMD \\ \cline{2-3}
	                          & Company (P)  & PMP, PMDMP, PMCMP \\ \cline{2-3}
	                          & Country (T)  & TMT, TMDMT, TMCMT \\ \cline{2-3}
	                          & Keyword (K)  & KMK, KMDMK, KMCMK \\ \cline{2-3}
	                          & Genre (G)    & GMG, GMDMG, GMCMG  \\ \hline

	\multirow{4}{*}{DBLP}                      & Paper (P)   & PAP, PTP \\ \cline{2-3}
	                          & Author (A)  & APA, APTPA \\  \cline{2-3}
	                          & Term(T)     & TPT, TPAPT \\ \cline{2-3}
	                          & Venue(V)    & VPV, VPAPV \\\specialrule{.1em}{0em}{0em}

	\end{tabular}
}
\vspace{-8pt}
\caption{ Metapaths used for each dataset.}
\label{tab:metapath}
\end{table}




==> sections/tables/notation.tex <==
\begin{table}[t]
\fontsize{8}{9} \selectfont
\centering
\caption{Notation Table.}
\vspace{-8pt}
\label{tab:notation}
\setlength{\tabcolsep}{1.0mm}{
	\begin{tabular}{c|p{6cm}}
	\specialrule{.1em}{0em}{0em}
	Notation  & Meaning   \\ \specialrule{.1em}{0em}{0em}
	$\mathcal{H}=(\mathcal{V}, \mathcal{E})$     & An HIN with node and edge sets  \\  \cline{1-2}
	$\phi: \mathcal{V} \rightarrow \mathcal{A}$	 & Map function of node type	\\  \cline{1-2}
	$\psi: \mathcal{E} \rightarrow \mathcal{R}$   & Map function of edge type	\\	\cline{1-2}
	$f^*$		& Optimal transport plan \\ \cline{1-2}
	$F$			& Cumulative distribution function \\ \cline{1-2}
	$g$			& node importance estimation function \\ \cline{1-2}
	$P_i$	& Abstracted feature distribution of $v_i$  \\ \cline{1-2}
 	$P_0$	& Reference distribution of $v_i$  \\ \cline{1-2}
	$v_i$, $e_i$ & node $v_i$ and edge between ($v_i$, $v_{i+1}$) \\ \cline{1-2} 
	$G_k^j=(\mathcal{V}_k^j, \mathcal{E}_k^j)$ &  Sub-network induced by $k$-th metapath \\ \cline{1-2}
	$\mathcal{V}_k^j$ & Node set with the $j$-th node type \\ \cline{1-2}
	$\mathcal{E}_k^j$  & Set of edges between nodes in $\mathcal{V}^j$ \\ \cline{1-2}
	$\mathbf{c}_{i, k}^{(l)}$  & $l$-th structural knowledge embedding of node $v_i$  \\ \cline{1-2}
	$\mathbf{f}_{i, k}^{att}$ & Attribute-aware similarity embedding \\ \cline{1-2}
	$\mathbf{f}_{i, k}^{top}$ & Topology-aware similarity embedding \\ \cline{1-2}
	$\alpha_{i, k}^{(l)}$ & Coefficient for $l$-th knowledge embedding \\ \cline{1-2}
 	$\widehat{\alpha}_{i, k}^{(l)}$ & Normalized coefficients \\ \cline{1-2} 
 	$\mathbf{e}_{i, k}$ & knowledge embedding derived for $k$-th metapath \\ \cline{1-2}
 	$\tau_{i, k}$ & Coefficient derived for $k$-th metapath  \\ \cline{1-2}
 	$\widehat{\tau}_{i, k}$ & Normalized coefficient \\ \cline{1-2}
 	$\mathbf{e}_i$ & Knowledge embedding of node $v_i$ \\ \cline{1-2}
 	$\mathbf{e}'_i$ & Initial feature of node $v_i$ \\ \cline{1-2}
 	$\mathbf{x}_i = [\mathbf{e}'_i, \mathbf{e}_i]$ & Aggregated embedding of node $v_i$ \\ \cline{1-2}
 	$\mathbf{h}_i^r$ & Hidden embedding learn by the $r$-th layer \\ \cline{1-2}
 	$\mathbf{q}_{i,m}^{(r)}$, $\mathbf{k}_{i,m}^{(r)}$, $\mathbf{v}_{i,m}^{(r)}$ & Query, key, value computation embeddings \\ \cline{1-2}
 	$S_m^{(r)}(v_j, v_i)$ & Attentive coefficient between nodes $v_j$ and $v_i$ \\ \cline{1-2}
 	$\tilde{\mathbf v}_{i,m}^{(r)}$ & Embedding with aggregated adjacent information  \\ \cline{1-2}
 	${\mathbf h}_i^{R}$ & Feature distribution representation of $v_i$ \\ \cline{1-2}
 	$\pi(\cdot)$ & Ranking indicator \\ \cline{1-2}
 	${\mathbf h}_i^{*}$ & Final representation of node $v_i$ \\ \cline{1-2}
 	$\mathcal{L}_{mse}$, $\mathcal{L}$ & Mean squared error loss and final objective \\  \specialrule{.1em}{0em}{0em}
	\end{tabular}
}
\end{table}

